Safe Bayesian Optimization using Interior-Point Methods -- Applied to Personalized Insulin Dose Guidance

This paper considers the problem of Bayesian optimization for systems with safety-critical constraints, where both the objective function and the constraints are unknown, but can be observed by querying the system. In safety-critical applications, querying the system at an infeasible point can have catastrophic consequences. Such systems require a safe learning framework, such that the performance objective can be optimized while satisfying the safety-critical constraints with high probability. In this paper we propose a safe Bayesian optimization framework that ensures that the points queried are always in the interior of the partially revealed safe region, thereby guaranteeing constraint satisfaction with high probability. The proposed interior-point Bayesian optimization framework can be used with any acquisition function, making it broadly applicable. The performance of the proposed method is demonstrated using a personalized insulin dosing application for patients with type 1 diabetes.

==> background.tex <==
\section{Background and related work}\label{sec:background}
\subsection{Gaussian processes}
Gaussian processes are popular nonparametric models that can be used to learn a nonlinear mapping $ f(x): \mathcal{X} \rightarrow \mathbb{R} $ from empirical data. This is done by assuming that $ f(x) $ is a random variable for any $ x \in \mathcal{X} $, and finite number of  these random variables have a joint Gaussian distribution \cite{rasmussen2006gaussian}. Gaussian processes are specified by its  mean and covariance function 
\begin{align*}
\mu(x)& := \mathbb{E}[f(x)]\\
k(x,x')&: = \mathbb{E}[(f(x)-\mu(x))(f(x')-\mu(x'))]
\end{align*}
Given the noisy observations $ y= f(x) + \omega $, with $ \omega  \sim \mathcal{N}(0,v^2)$,  we can predict the function value at an arbitrary point $ x_{*} \in \mathcal{X}$ by conditioning the joint Gaussian prior distribution on the observations $ \{(x_{0},y_{0}), \dots, (x_{n-1},y_{n-1})\}$. This gives the posterior distribution with mean and variance
\begin{subequations}\label{Eq:GPconditioning}
\begin{align}
	\mu(x_{*})& = \mathbf{k}(x_{*}) ^{\mathsf{T}}(\mathbf{K} + v^2\mathbf{I})^{-1}\mathbf{y}\\
	\sigma^2(x^*) &= k(x_{*},x_{*}) - \mathbf{k}(x_{*})^{\mathsf{T}}(\mathbf{K} + v^2 \mathbf{I})^{-1}\mathbf{k}(x_{*})
\end{align}
\end{subequations}
where $\mathbf{y} = [y_{0}, \dots, y_{n-1}]^{\mathsf{T}}$ are the observations, $ \mathbf{k}(x_{*}) = [ k(x_{*},x_{0}),\dots,k(x_{*},x_{n-1})] $ is the covariance between $ x_{*} $ and the observed inputs $ [x_{0}, \dots, x_{n-1}]^{\mathsf{T}} $,  $ \mathbf{K} \in \mathbb{R}^{n\times n} $  is the covariance matrix with entries $ \mathbf{K}_{(i,j)} = k(x_{i},x_{j}) $ for $ i,j \in \{0,\dots,n-1\} $ \cite{rasmussen2006gaussian}.


\subsection{Bayesian optimization}
\noindent For an unconstrained optimization problem $
\min_{x\in\mathcal{X}} f^{0}(x) $,
Bayesian optimization places a probabilistic surrogate model, typically a Gaussian process, to best represent our belief about the unknown cost function $ f^0(x)$ given the observations $ \{(x_{i},y_i)\}_{i=0}^{n-1} $. Using the updated probabilistic surrogate model, at each iteration we compute the next query point $ x_{n} \in \mathcal{X}$ to be evaluated. The choice of the next query point is a crucial step since it must trade-off exploration and exploitation to find the optimum in as few iterations as possible. This is done by using  acquisition functions $ \alpha^0: \mathcal{X} \rightarrow \mathbb{R} $ (also known as utility functions or infill functions)   that are induced from the updated probabilistic surrogate model \cite{mockus1978application,jones1998efficient}. That is,
\begin{equation}\label{Eq:BayesOptIntro2}
	x_{n} = \arg \min_{x\in\mathcal{X}} \alpha^0(x)
\end{equation}
There are many choices for an acquisition function. For example,  improvement-based policies such as probability of improvement \cite{kushner1964new} and expected improvement \cite{mockus1978application} encourage points that are likely to improve over the best observed point. Optimistic policies such as GP-LCB\footnote{Commonly referred to as GP-UCB for maximization problems in the Bayesian optimization literature.} encourages points that  optimistically lead to the minimum \cite{srinivas2009gaussian}. Information-based policies such as Thompson sampling \cite{thompson1933likelihood,chapelle2011empirical} and entropy-search \cite{hennig2012entropy} are based on the posterior distribution over the unknown minimizer. 
The newly evaluated data point $ \{x_{n},y_{n}\} $ is then appended to the data set, and the process is repeated. 


\subsection{Constrained Bayesian optimization}
If the constraints are known \textit{a priori}, then this can be used to determine the feasible action space $ \mathcal{F} \subseteq \mathcal{X} $. However, the challenging case arises when the constraints are  unknown, since in this case $  \mathcal{F} $ is unknown. In constrained Bayesian optimization literature, this is typically handled by placing  probabilistic surrogate models for each constraint in addition to the cost function, which are updated based on the noisy observations of the constraints.   

%Depending on whether the constraints are safety-critical or not, there are two classes of constrained Bayesian optimization. The first class of problem deals with a  sequential search algorithm using the scaled acquisition function, during which the constraints may be violated. After some number of queries (typically when the budget is exhausted), the algorithm makes a final recommendation of the solution.
 % The second class of problem deals with safe learning, where the constraints must be feasible through out the sequential search. 

Initial works in the direction of constrained Bayesian optimization such as  \cite{gelbart2014constrained,gardner2014bayesian} handled the constraints by scaling the acquisition function  with the probability of constraint feasibility
\begin{equation}\label{Eq:PF}
	x_{n} = \arg \min_{x \in \mathcal{X}}  \prod_{i=1}^m \Phi^{i}(x)\alpha^0(x)
\end{equation}
where $ \Phi^{i}(x)  $ is the cumulative density function of the $ i^{th} $ constraint GP \cite{gelbart2014constrained}. However, in this approach, the next query point may violate the constraints since the probability of feasibility is only known accurately after observing a data point. This approach  is therefore not suitable when we have safety-critical constraints.


In the presence of safety-critical constraints,% optimizing an objective function with partially revealed constraints are complicated, since explorations can be performed only within the feasible set, which is unknown. Simply put, 
 it is highly undesirable to explore an action where the safety-critical constraints would be violated. Hence, one has to carefully choose the next query point, such that the safety-critical constraints are satisfied with high probability. The authors in \cite{sui2015safe} presented the SafeOPT algorithm, where the safety-critical constraints were posed as a minimum performance requirement constraint. This was later extended to the case with arbitrary safety constraints decoupled from the performance objective in \cite{berkenkamp2021bayesian}. These approaches are based on identifying a safe set based on the constraint observations. The safe set in these approaches are enlarged using  Lipschitz continuity properties.%, which unfortunately is often not easily known for many applications in practice. 

The authors in \cite{pourmohamad2021bayesian} recently presented a Bayesian optimization approach using barrier functions, where the barrier functions are incorporated into the Gaussian process models itself, and the authors proposed modified acquisition functions. However, this approach has some practical challenges.  Firstly, such an approach does not guarantee constraint feasibility with high probability. Secondly, their approach also involves computing the expectation of the log operator which is not trivial to compute. Thirdly, this approach requires the use of the specific acquisition function proposed in \cite{pourmohamad2021bayesian} that is based on approximating the expectation of the log operator.  %
% \paragraph{Contextual Bayesian optimization}
% 


%Many applications also have safety critical constraints that need to be satisfied. % Safey critical applications where the constraints cannot be violated. 



% In the literature, there is Bayesian optimization with constraints, where he acqusiion funcion is scaled using the probability of feasibility. Here, the algorithm converges to a solution, where the constraints are feasible, but can pottentially explore actions that would  violate the constraints. 
% Such methods are not suited for safety critical applications, since the constrraints must not be violated even when exploring. 
% this lead to the development of Safe BayesOpt by Sui et al.. where the constraints are on the objective functon itself. This was later extended to the case where tthe constraints are not just on the cost by beerkenkamp. These appraoches are based on iddentifying a safe-set witthin which the the next query point lies. This allowed the authors to develop a safe learning strategy. After each query point, the safe sets were updated based on the Lipschitz continuity of the function, which may not be practically available in some applications. 

% In this paper, we propose a safe exploration strategy by using the Barrier mthod. In particualt, we add a Barrier penalty term in the acqusition function based on the lower confidence bound of the constraint GP. 

% Note that this method is different from the work of .... where they also consider a barrier method, but the barrrier method is based on the mean... something that is not correct, and does not gurantee constraint feasibiltiy with high probability. But a major drawback of this approach is that it requres a particular acqusiition fgunction that the authors develop, and cannot be used with the other acquitiison function. 

% Compared to this work, our proposed method firstly can be used with any acqusiotion function, and the secondly, can gurantee constraint feasibilirt with high proabability. 


\subsection{Contributions}
This paper focuses on the  problem of safe learning, and proposes an algorithm for safe Bayesian optimization using interior-point methods that guarantee constraint satisfaction with high probability. The approach is similar to that of the \cite{berkenkamp2021bayesian}, however, instead of using the Lipschitz continuity properties to identify the safe set at each iteration, we enforce constraint by using additional log-barrier terms.  Unlike the approach in \cite{pourmohamad2021bayesian}, we propose to add the log-barrier terms only in the acquisition function. This makes our applicable with any acquisition function to find the optimum, and also ensures constraint satisfaction with high probability. Moreover, we also avoid taking expectation of the log-operator in our approach.

The proposed safe Bayesian optimization is then used to develop a personalized  insulin dose guidance algorithm  for patients with type 1 diabetes, where we show that we can find the optimum insulin dose for each patient in a few iterations without violating the safety-critical constraints. The performance of the approach is demonstrated on the US-FDA approved UVA/Padova virtual patient simulator.%, as well as the virtual patient simulator based on the T1D-Hovorka model.

% One such application area is Personalized medicine. Finding the optimal drug dose can be challenging, since the effect of the drug can vary a lot from one individual to the other. Often times there are several factors that impac the eficiacy of a drug, such as age, gender, boddy mass, metabolism, other underlying conditions, etc.... As such, models developed based on a population level are hence not well suited for optimal drug dosing in each individual.  it is impossible to assume access to models that are personlized to each individual. 
% In this paper we will demonstrate the performance of the proposed approach on optimal insulin dosing problem to counteract the effect of meal consumption.

%% Takee some text from the proposal document. 

